Semi-parametric dynamic contextual pricing

Motivated by the application of real-time pricing in e-commerce platforms, we consider the problem of revenue-maximization in a setting where the seller can leverage contextual information describing the customer's history and the product's type to predict her valuation of the product. However, her true valuation is unobservable to the seller, only binary outcome in the form of success-failure of a transaction is observed. Unlike in usual contextual bandit settings, the optimal price/arm given a covariate in our setting is sensitive to the detailed characteristics of the residual uncertainty distribution. We develop a semi-parametric model in which the residual distribution is non-parametric and provide the first algorithm which learns both regression parameters and residual distribution with $\tilde O(\sqrt{n})$ regret. We empirically test a scalable implementation of our algorithm and observe good performance.

==> conclusions.tex <==
% !TEX root = root.tex

\section{Conclusion and Extensions}

In this paper we develop a pricing algorithm which leverages covariates  and achieves optimal regret scaling in time horizon $n$. We characterize its scaling with respect to covariate dimension $d$ via a small set of parameters which characterize compactness and smoothness of the underlying distributions. 

Further, some of our assumptions can be relaxed as we briefly describe below. 

%\subsection{Scaling w.r.t.\ covariate dimension $d$}

\subsection{Relaxing compactness of support of covariates}
We believe that the compactness assumption of $\mathcal X$ in A\ref{Assumption:IID_XZ} can be significantly relaxed. For example, consider the following simple relaxation. (We say that a random variable $W$ is $\sigma$-subgaussian if $\P(X>t) \le e^{-\sigma^2t^2}$.)


\begin{assumption}\label{assumption:SubgaussianXZ}
$\{X_t\}_t$ and $\{Z_t\}_t$ are i.i.d.\ and mutually independent. Their distributions are unknown to the platform. The support of $Z_1$, namely $\mathcal{Z}$, is compact and known. Let
$$W = \sup_{z\in \mathcal Z, \theta \in \Theta} ze^{\theta^\intercal X_1}.$$
$W$ is $\sigma$-subgaussian for a known $\sigma >0$. 
\end{assumption}

 Under A\ref{Assumption:Theta}, and A\ref{Assumption:Kappas}, and A\ref{assumption:SubgaussianXZ} we can obtain a result analogous to Theorem~\ref{thm:RegretBound} as follows. 

Recall that the policy DEEP-C requires knowledge of $\alpha_2$, which in this case may be infinity. However, the platform can compute $\alpha'_2$ such that $P(W > \alpha'_2) \le 1/n^2$, and execute policy DEEP-C with $\alpha'_2$ instead of $\alpha_2$. Thus, the probability of event $\{\exists t \in \{1,\ldots,n\} V_t > \alpha'_2\}$ is at most $1/n$, and the overall impact of such an event on expected regret is $O(1)$. Using the fact that, since $\mathcal{Z}$ and $\Theta$ are compact, there exists $\alpha'_1 >0$ (possibly unknown to the platform) such that $P(W < \alpha'_2) \le 1/n^2$, we can obtain a regret bound similar to Theorem~\ref{thm:RegretBound}.  


\subsection{Incorporating adversarial covariates} 

We believe that the i.i.d.\ assumption on covariates can also be significantly relaxed. As a prelude, consider the following modification to A\ref{Assumption:IID_XZ}.

\begin{assumption}\label{assumption:AdversarialCovariates}
 We assume that $\{Z_t\}_t$ are i.i.d.\ with compact support $\mathcal Z$. We assume that the support of $X_t$ for each $t$ is compact, namely $\mathcal X$.  Given the past, $X_t$ can be chosen adversarially from its support. More formally, we assume that $\mathcal X$ is $\sigma(X_1,\ldots,X_{t-1},Z_1, \ldots, Z_{t-1}, p_1,\ldots, p_{t-1})$-measurable. 
  \end{assumption}
  
%Note that, since $Y_t$ is a function of $X_t$, $Z_t$, and $p_t$, thus the above $\sigma$ algebra includes $\sigma(Y_1,\ldots,Y_{t-1})$ as well. 
Given Assumption A\ref{assumption:AdversarialCovariates}, consider the following strengthening of Assumption A\ref{Assumption:Kappas}.  Recall that $F(z) = z \P(Z_1>z)$. Let  
$$r(z,\theta, x) = e^{\theta_0^\intercal x} F\left(e^{-\left(\theta_0-\theta \right)^\intercal x} z\right).$$
%
Given covariate $x$, $r(z,\theta,x)$ can be viewed as the expected revenue at $(z,\theta)$.
%Let $\theta^{(l)}$ represent the $\l\kth$ component of $\theta$, i.e., $\theta = (\theta^{(l)}: 1\le l \le d)$. 

\begin{assumption}\label{assumption:LocalConcavity_Adversarial}
We assume that there exist $\kappa_1,\kappa_2 >0$ such that for each $z \in \mathcal{Z}$, $\theta \in \Theta$, and $x \in \mathcal X$ we have
$$ \kappa_1(z^* - z)^2 \le r(z^*, \theta_0,x) - r(z,\theta,x) \le \kappa_2(z^* - z)^2 , $$
and for each $1\le l \le d$,
$$ \kappa_1(\theta_0^{(l)} - \theta^{(l)})^2 \le r(z^*, \theta_0,x) - r(z,\theta,x) \le \kappa_2(\theta_0^{(l)} - \theta^{(l)})^2 . $$
\end{assumption}

We conjecture that under assumptions A\ref{assumption:AdversarialCovariates}, A\ref{Assumption:Theta}, and A\ref{assumption:LocalConcavity_Adversarial}, a suitable modification of DEEP-C Policy would achieve a regret scaling similar to (if not the same as) that in Theorem~\ref{thm:RegretBound}. This conjecture rests on the following two key observations: (1) The optimal policy for the \Oracle{} with adversarial covariates is the same as that under the i.i.d.\ covariates setting; and (2) the DEEP-C policy for i.i.d.\ covariates does not learn or use the distribution of $X_t$ (except via the knowledge of the support, and the constants $\alpha_2,\kappa_1$ and $\kappa_2$). %We plan to pursue this extension in the near future. 



%\subsection{Leveraging sparsity} 
%In this paper we focussed on 

